Challenges and Opportunities in Offline Reinforcement Learning from Visual Observations

Offline reinforcement learning has shown great promise in leveraging large pre-collected datasets for policy learning, allowing agents to forgo often-expensive online data collection. However, offline reinforcement learning from visual observations with continuous action spaces remains under-explored, with a limited understanding of the key challenges in this complex domain. In this paper, we establish simple baselines for continuous control in the visual domain and introduce a suite of benchmarking tasks for offline reinforcement learning from visual observations designed to better represent the data distributions present in real-world offline RL problems and guided by a set of desiderata for offline RL from visual observations, including robustness to visual distractions and visually identifiable changes in dynamics. Using this suite of benchmarking tasks, we show that simple modifications to two popular vision-based online reinforcement learning algorithms, DreamerV2 and DrQ-v2, suffice to outperform existing offline RL methods and establish competitive baselines for continuous control in the visual domain. We rigorously evaluate these algorithms and perform an empirical evaluation of the differences between state-of-the-art model-based and model-free offline RL methods for continuous control from visual observations. All code and data used in this evaluation are open-sourced to facilitate progress in this domain.

==> 08_ack.tex <==
\begin{ack}
Cong Lu and Tim G. J. Rudner are funded by the Engineering and Physical Sciences Research Council (EPSRC).
Philip J. Ball is funded through the Willowgrove Studentship.
Tim G. J. Rudner is also funded by the Rhodes Trust and by a Qualcomm Innovation Fellowship.
We are grateful to Rafael Rafailov for sharing the data used with LOMPO and Edoardo Cetin for his NumPy Array replay buffer implementation.
We thank Samuel Daulton, Clare Lyle, Muhammad Faaiz Taufiq for detailed feedback on an early draft.
The authors would also like to thank the anonymous ICML 2022 and NeurIPS 2022 reviewers for constructive feedback which helped improve the paper.
\end{ack}

